Domain Specialization as the Key to Make Large Language Models Disruptive: A Comprehensive Survey

Large language models (LLMs) have significantly advanced the field of natural language processing (NLP), providing a highly useful, task-agnostic foundation for a wide range of applications. However, directly applying LLMs to solve sophisticated problems in specific domains meets many hurdles, caused by the heterogeneity of domain data, the sophistication of domain knowledge, the uniqueness of domain objectives, and the diversity of the constraints (e.g., various social norms, cultural conformity, religious beliefs, and ethical standards in the domain applications). Domain specification techniques are key to make large language models disruptive in many applications. Specifically, to solve these hurdles, there has been a notable increase in research and practices conducted in recent years on the domain specialization of LLMs. This emerging field of study, with its substantial potential for impact, necessitates a comprehensive and systematic review to better summarize and guide ongoing work in this area. In this article, we present a comprehensive survey on domain specification techniques for large language models, an emerging direction critical for large language model applications. First, we propose a systematic taxonomy that categorizes the LLM domain-specialization techniques based on the accessibility to LLMs and summarizes the framework for all the subcategories as well as their relations and differences to each other. Second, we present an extensive taxonomy of critical application domains that can benefit dramatically from specialized LLMs, discussing their practical significance and open challenges. Last, we offer our insights into the current research status and future trends in this area.

==> Chapters-tex/application.tex <==
%Nature Science or Social Science: nature science can include health, chemistry, physics, climate, environment, software (programming language), etc., those more scientific disciplines or sub-fields; then social science can include education, finance (business), law, humanity, policy-making (public health), etc.
% avoid BERT, GPT2
% 2020-2023

\subsection{Biomedicine}
\noindent Language models are becoming increasingly useful in the field of biology, from fundamental biomedical research to clinical healthcare support. At the fundamental biomedicine science level, LLMs can be trained on vast amounts of domain-specializing data (e.g., genomic and proteomic) to analyze and predict biological functions, disease mechanisms, and drug discovery. LLMs can also aid in predicting protein structures and interactions, which are critical for understanding cellular processes and designing new drugs. At the clinical healthcare support level, pre-trained or medical corpus fine-tuned LLMs can be used for the natural language processing of medical records to identify patterns, make diagnoses, and provide personalized treatment recommendations. Also, LLMs can assist in medical image analysis in a multi-modality learning way, such as identifying specific features in X-rays or MRI scans. Overall, LLMs offer tremendous potential for advancing biology research and improving healthcare outcomes.

\subsubsection{Fundamental Biomedicine Science}
% \noindent\textbf{Molecular biology} 
Recent advancements in LLMs have provided promising results in fundamental biomedical research~\cite{mahjour2023designing}. These models allow for the integration of diverse data sources, such as molecular structures, genomics, proteomics, and metabolic pathways, enabling a more comprehensive understanding of biological systems. Several application-specific LLMs have been developed for molecular and biological sciences.
For instance, MoLFormer~\cite{ross2022large} is a large-scale molecular SMILES transformer model with relative position embedding that enables the encoding of spatial information in molecules. 
Nucleotide Transformer~\cite{dalla2023nucleotide} is a foundation model pre-trained on DNA sequences for accurate molecular phenotype prediction, essentially treating single amino acids or stretches of k-memorized DNA as words in a vocabulary and using LLMs to learn from the biological sequences.  
ESM-2 and ESMFold are transformer protein language models included in the Evolutional Scale Modeling (ESM) family~\cite{rives2021biological}, which can generate accurate structure predictions directly from a protein's sequence and outperform other single-sequence protein language models. 
ProtGPT2~\cite{ferruz2022protgpt2} is a language model trained on the protein space that generates de novo protein sequences following the natural principles. ProGen~\cite{madani2023large} is a deep-learning language model that can generate protein sequences with predictable functions across large protein families. Artificial proteins fine-tuned to distinct lysozyme families using ProGen have shown similar catalytic efficiencies as natural proteins with low sequence identity.

% \noindent\textbf{Pharmacy research} involves discovering new chemical compounds that have the potential to treat or alleviate human ailments effectively. 

\subsubsection{Clinical Healthcare Support}
% \noindent\textbf{Medical texts and EHR analysis} 
LLMs have greatly assisted in medical text and electronic health records understanding, leading to a range of potential benefits for healthcare~\cite{rao2023evaluating, jeblick2022chatgpt, moons2023chatgpt, rao2023assessing, nastasi2023does, zuccon2023dr, antaki2023evaluating}. 
Recently, there have been several major domain-specific LLMs developed for various NLP tasks in the biomedical domains. BioGPT \cite{luo2022biogpt} is a domain-specific generative Transformer language model pre-trained on large-scale biomedical literature, which achieves impressive results on most biomedical NLP tasks spanning document classification, relation extraction, question answering, etc. 
BioMedLM \cite{BioMedLM} is another state-of-the-art GPT-style language model trained on biomedical literature from The Pile\footnote{https://pile.eleuther.ai/}, capable of achieving high accuracy on various biomedical NLP tasks, including MedQA, and possesses language generation capabilities, developed for research purposes to advance the development of biomedical NLP applications and responsible training and utilization of domain-specific language models.
\cite{tang2023does} explore the utilization of LLM synthetic data for clinical text mining. Med-PaLM~\cite{singhal2022large} also generates accurate, helpful long-form answers to consumer health questions, as judged by panels of physicians and users, which helps in treatment recommendations to suggest customized medications to patients based on their unique health circumstances. This can assist physicians in selecting the most efficient drugs for their patients, ultimately enhancing treatment outcomes. GatorTron~\cite{yang2022gatortron} are models from scratch using the BERT architecture of different sizes on a large corpus consisting of over 90 billion words from clinical narratives, and scientific literature. \cite{yang2022large} further developed a GatorTro model from scratch on learning unstructured electronic health records. % Earlier, the PubMedBERT~\cite{gu2021domain} is pre-trained from scratch using abstracts from PubMed, which once achieved state-of-the-art performance on several biomedical NLP tasks on the Biomedical Language Understanding and Reasoning Benchmark.
Besides, LLMs can also directly help to anticipate the potential illnesses that a patient may develop based on their past medical history. For example, Med-BERT~\cite{rasmy2021med} produces pre-trained contextualized embeddings on large-scale structured electronic health records for disease prediction. 
ChatCAD~\cite{wang2023chatcad} proposes a method for integrating LLMs into medical-image Computer-Aided Diagnosis (CAD) networks with the goal of creating a more user-friendly system for patients and improving CAD performance. 
LLM also brings opportunities and challenges for domain educators or policymakers~\cite{kung2023performance, fijavcko2023can, wang2023chatgpt, kortemeyer2023could, sifat2023chatgpt}. On public health informatics, the use of LLMs can also help in analyzing the conversations about the impact of the COVID-19 pandemic on societies worldwide~\cite{sallam2023chatgpt}, which are taking place on social media platforms such as Twitter~\cite{chen2020tracking}.

\subsubsection{Future Research Opportunities}
In biomedicine domain, the utilization of LLMs faces significant challenges due to the scarcity of high-quality labeled data. The complexity and heterogeneity of biomedical data across different tasks make proper annotation time-consuming and expensive, requiring domain-specific expertise~\cite{lehman2023CLM}. LLMs trained on specific biomedical datasets may lack generalizability to diverse patient populations and clinical contexts. Hallucination, the generation of inaccurate or incorrect information, is a major concern with LLMs in biomedicine, which can lead to harmful errors in real-world applications~\cite{beutel2023artificial, azaria2023internal}. For instance, false-positive relationships between drugs and diseases in biomedical literature-trained LLMs can result in incorrect treatment recommendations or adverse effects~\cite{lee2023benefits}. Despite these challenges, the use of LLMs in biomedicine offers promising opportunities for research and clinical practice. Recent studies demonstrate that LLMs like GPT-3 can effectively capture the semantics and context of biomedical language, facilitating more accurate representation of biomedical knowledge~\cite{agrawal2022large, singhal2022large, nath2022new}. LLMs enable integration and analysis of diverse biomedical data sources, supporting the development of precise medical ontologies and taxonomies~\cite{lu23HiPrompt}. They also enable the identification of new phenotypic and genotypic correlations and the discovery of novel drug targets. To mitigate the risk of generating inaccurate information, various approaches can be employed, such as utilizing curated datasets, implementing sampling-based self-check methods~\cite{manakul2023selfcheckgpt}, conducting causality analysis~\cite{arsenyan2023large}, and incorporating external knowledge to enhance LLMs~\cite{peng2023check}. By addressing these challenges and leveraging the strengths of LLMs, the use of LLMs in biomedicine can revolutionize healthcare delivery and improve patient outcomes.

\subsection{Earth Science}
Earth science is an interdisciplinary domain focused on examining the interactions between physical and human systems across diverse spatial and temporal scales. This field incorporates methods from Earth observation, information science, spatial analysis, complexity theory, and simulation modeling to investigate phenomena like climate change, land-use change, natural disasters, environmental development, and urbanization. Spatial information is vital to Earth science, and geographic information science tools are invaluable for a wide range of interdisciplinary studies involving spatial data. Large language models like ChatGPT can act as question-answer systems, assisting those interested in Earth Science to gain pertinent knowledge, such as recommending the optimal earth observation dataset for specific research purposes, offering code examples like Google Earth Engine code for processing satellite data, providing high-quality responses to environmental-related questions \cite{zhu2023chatgpt}, developing innovative idea \cite{biswas2023potential}, generating climate scenario \cite{biswas2023potential}. LLMs can also be tailored to various Earth Science-related downstream tasks through methods such as fine-tuning, few-shot, or even zero-shot learning. 

\subsubsection{Geospatial Semantic Tasks}
A study \cite{mai2022towards} evaluated GPT-2 and GPT-3 on two geospatial semantic tasks: toponym identification and location description recognition. The former task involves detecting named locations within a given text snippet, and the latter entails identifying more detailed location descriptions, like home addresses, highways, roads, and administrative regions, from a text snippet such as tweets. The findings suggest that task-agnostic LLMs can surpass task-specific, fully-supervised models in both tasks, with sigificant improvement in few-shot learning scenarios. Moreover, \cite{mai2023opportunities} broadened this comparison by incorporating four differently-sized pre-trained GPT-2 models, the latest GPT-3, InstructGPT, and ChatGPT, as well as various supervised, task-specific benchmarks for the same two representative geospatial semantic tasks. The outcomes showed that LLMs, with only a limited number of few-shot samples, can outperform fully supervised, task-specific models in well-defined geospatial semantic tasks. This underscores the potential of LLMs to considerably lessen the reliance on custom architectures or extensive labeled datasets for geospatial semantic tasks. However, further research is necessary to determine the most effective ways to create appropriate prompts for guiding LLMs in specific geospatial semantic tasks.

\subsubsection{Spatial Classification and Time-Series Forecasting}
LLMs are increasingly used for various geospatial artificial intelligence tasks, including classification and time series forecasting, through a prompt-based learning approach. In a study by Mai et al. \cite{mai2023opportunities}, the frequencies of different types of Point of Interest (POIs) within an urban region were transformed into a textual paragraph. The researchers employed LLMs to predict the urban function of the region based on this paragraph. The study compared GPT2, GPT-3, and ChatGPT models under zero-shot and one-shot settings with two supervised learning neural networks. The results indicated that ChatGPT exhibited superior precision and recall compared to other GPT models. Another example is PromptCast \cite{xuepromptcast}, a prompt-based time series forecasting model. The authors conducted forecasting on three real-world datasets: city-temperature data, safe graph human mobility, and electricity consumption load data. The findings in both single- and multi-step forecasting settings demonstrated the potential of prompt-based time series forecasting with language generation models. Moreover, PromptCast exhibited better generalization ability in the zero-shot setting compared to conventional numerical-based forecasting. Additionally, Mai et al. \cite{mai2023opportunities} utilized LLMs to forecast the number of deaths due to dementia in different geographic regions, including state and county levels.

\subsubsection{Text-Guided Earth Observation Image Processing}
LLMs enable multimodal analysis, integrating text, audio, images, and videos with other foundation models like vision models. In a study by Mai et al. \cite{mai2023opportunities}, VLFMs (OpenCLIP, BLIP, and OpenFlamingo-9B) were employed for an urban perception task using a street view image noise intensity dataset. While most VLFMs faced challenges in connecting visual features to nuanced semantics and concepts in urban studies, BLIP demonstrated balanced and reasonable predictions, comparable to fine-tuned CNN models. VLFMs can comprehend certain characteristics of urban neighborhoods from visual inputs, but their language-only abilities are not as strong as LLMs. Zhang et al. \cite{zhang2023text2seg} developed Text2Seg, a pipeline that facilitates remote sensing image semantic segmentation tasks using text prompts. The pipeline incorporates three methods: Grounding DINO generates bounding boxes from a text prompt, which are used in SAM to create a segmentation map; CLIP Surgery produces a heat map from a text prompt, sampled to create point prompts for SAM to generate segmentation masks; and SAM generates multiple segmentation maps, compared to the semantic similarity of the text prompt using CLIP. The initial assessment highlighted the benefits of integrating multiple foundation models in a single pipeline \cite{zhang2023text2seg,mai2023opportunities}.

\subsubsection{Future Research Opportunities}
Although LLMs have shown promise in some language-only geospatial tasks as zero-shot or few-shot learners, they have also been criticized for generating inaccurate and misleading results. This issue is particularly problematic in a geographic context, where generating geographic faithful results is crucial for nearly all GeoAI tasks \cite{mai2023opportunities}. LLMs face challenges in more complex geospatial semantics tasks, such as toponym resolution/geoparsing and geographic question answering, as they are unable to conduct implicit spatial reasoning grounded in the real world. Additionally, integrating LLMs with other foundation models to perform tasks involving multiple data modalities remains a significant challenge in this field.   


\subsection{Finance}

\noindent Utilization of NLP technologies in the financial industry, especially the fintech domain, is wide and growing\cite{xing2018natural} \cite{fisher2016natural}. Common NLP tasks in the trading and investment management domain include sentiment analysis \cite{souma2019enhanced}, question answering with generative language model \cite{wang2022novel}, named entity recognition (NER) \cite{alvarado2015domain}, text classification \cite{zhao2020study}. 


\subsubsection{Sentiment Analysis Task in Finance} 

The value of financial instruments is often influenced by public information about the underlying entities. Various forms of financial texts, such as news articles, analyst reports, and SEC filings, are all potential sources of new information that could affect market prices. As a result, the use of NLP techniques for sentiment analysis to predict price movements and returns has become increasingly popular in recent years \cite{chowdhury2014news}.

FinBERT, a fine-tuned BERT model for finance, has emerged as a useful tool for financial sentiment analysis. While the general BERT model has proven to be more effective than traditional dictionary-based approaches for financial sentiment analysis \cite{leippold2023sentiment}, FinBERT has been particularly useful for addressing the unique challenges posed by the specialist language used in financial contexts \cite{araci2019finbert}. The FinBERT model was pre-trained on a financial corpus and then fine-tuned specifically for sentiment analysis tasks, yielding significantly better results than previous state-of-the-art approaches. The ChatGPT model, a newer entrant to the field, has also shown promising results, outperforming BERT and earlier models such as GPT-1 and GPT-2 in studies on predicting stock prices using sentiment analysis of news headlines \cite{lopez2023can}. It has also been utilized to assess news outlet credibility \cite{yang2023large}, adding another dimension to its applications in the financial sector. Just like BERT, ChatGPT could encounter challenges when dealing with the specialist language used in finance, indicating a substantial opportunity for fine-tuning this model to make it a dominant tool for financial sentiment analysis tasks.
\subsubsection{Financial Data Generation}
Generative language models are found to be particularly helpful in sales and client engagement processes in the finance industry, either in consumer finance, insurance, or investment finance \cite{quah2019chatbot}. For example, financial institutions have deployed customer service chatbots to provide instant responses to customer inquiries. The Chatbots have mostly been developed with the general BERT model, seq2seq, word2vec or machine learning-based classification models with historical question and answer data \cite{wube2022text}. For financial products salespersons, generative language models are used widely to automate sales emails, build sales call agendas and summarize sales notes for client insights and discover product trends. With arising LLM, fine-tuned LLM with historical client inquiries data or domain financial contexts will be promising enhancements to current generative tasks in finance.

% \subsubsection{Others}
% NER task in the finance domain aims to retrieve financial entities (e.g., financial institutions, currencies, and companies) in financial texts. Fine-tuned pre-trained language models such as FinBERT-MRC \cite{zhang2023finbert} are increasingly popular in specific financial NER tasks. Another important NLP task is text classification. Sentiment analysis is essentially a sub-task in text classification. However, fine-tuned BERT model of FinBERT does not demonstrate superior performance than general BERT in classifying financial texts with model fine-tuning \cite{arslan2021comparison}.       

\subsubsection{Future Research Opportunities} 
% \noindent\textbf{finance} 
The release of GPT-3 sparked curiosity around its potential uses in various specific fields, such as tax consultancy \cite{bommarito2023gpt} and investment portfolio construction \cite{niszczota4384861gpt}. Initial assessments indicated that, while GPT-3 performed better than random guessing, it still fell short of human performance in these tasks. However, the debut of Bloomberg's domain-specific LLM, BloombergGPT, demonstrated significant improvements in performance on financial tasks without compromising its performance on general LLM benchmarks \cite{wu2023bloomberggpt}. This has fueled further interest in domain-specific LLMs in the finance field, prompting predictions of future development of models with similar capabilities, whether through training on specific financial data or fine-tuning existing models. Despite these promising results, the adoption of LLMs in finance is not without its challenges. Notably, data security and intellectual property concerns are of significant importance in this sector. Companies are rightfully apprehensive about the possibility of their proprietary data being leaked during the model training process. Furthermore, questions arise around the ownership of intellectual property when GPT-generated code is incorporated into commercial software products. As the field progresses, these concerns will need to be addressed to facilitate the wider application of LLMs in the financial sector.


\subsection{Law}
General PLMs have shown great promise in many NLP tasks, including in the legal domain. However, due to the intricate nature of legal language, these generic models might fall short \cite{chalkidis2020legal}. To improve accuracy in legal applications, Chalkidis et al. proposed LEGAL-BERT, trained specifically on legal corpora, resulting in enhanced legal text classification performance \cite{chalkidis2020legal}. Prasad et al. further showed that fine-tuning LEGAL-BERT can improve its effectiveness even in unfamiliar legal domains \cite{prasad2022effect}. Despite these improvements, Valvoda et al. cautioned that LEGAL-BERT might produce asymmetric predictions in legal outcomes, which could influence real-life legal decisions \cite{valvoda2023on}. These findings have driven NLP researchers to develop specialized language models such as LLMs for nuanced fields like law. Current efforts can be classified into two main categories: one focusing on LLM domain adaptation, such as legal prompting, and the other examining the transformative potential of LLMs in legal applications through empirical evaluations.\subsubsection{Legal Prompting}
LLMs, like GPT-3, have been explored for their potential in handling legal tasks, including statutory reasoning and legal judgment prediction. Legal prompting has been employed to guide and assist LLMs in these tasks, given its significance in the legal domain. For instance, Blair-Stanek et al. investigated the performance of GPT-3 on statutory reasoning using different instruction methods, including zero-shot prompting, few-shot prompting, and chain-of-thought prompting \cite{blair2023can}. The study revealed that chain-of-thought prompting achieved the highest accuracy, although legal reasoning techniques surpassed this by further enhancing accuracy \cite{blair2023can}. The researchers utilized templates and schemas to guide the reasoning process of GPT-3, resulting in improved accuracy in legal reasoning tasks \cite{blair2023can}.
Similar performance improvement was observed for legal judgment prediction. Yu et al. \cite{yu2022legal} used chain-of-thought prompting to guide the GPT-3 model and demonstrated improved performance on this task. Specifically, they provided GPT-3 with legal case summaries and asked it to predict the outcome of the case. The authors found that the model could accurately predict the outcome with the help of legal prompting. Recent work also \cite{trautmann2022legal} demonstrated that zero-shot legal prompt engineering performed better than all baselines, but fall short compared with supervised approaches.

%Overall, these studies highlight the potential of legal prompting to guide and assist LLMs in performing legal tasks with improved accuracy. Legal prompting not only helps the model perform better but also helps to ensure that the model is making decisions based on legal reasoning and principles.

\subsubsection{Legal Assessment}
The development of LLMs has attracted the attention of legal scholars who have explored their potential to revolutionize the legal field. One potential application of LLMs is to assist in legal education and preparation for law exams. Bommarito et al. \cite{bommarito2022gpt}, Choi et al. \cite{choi2023chatgpt}, and Katz et al. \cite{katz2023gpt} have conducted case studies to evaluate the performance of LLMs on law exams with the help of legal prompting. The results indicate that LLMs can achieve promising performance with the assistance of legal prompting. However, it is important to note that LLMs are not expected to replace lawyers in the legal profession. One limitation of LLMs in the legal domain is their difficulty in identifying recent case law due to outdated data sources. Macey et al. \cite{macey2023chatgpt1,macey2023chatgpt2} and Iu et al. \cite{iu2023chatgpt} discussed this issue and suggested that LLMs need to be trained on up-to-date legal databases to improve their performance in this area. 


\subsubsection{Future Research Opportunities}
The use of LLMs in the legal domain has shown promise, but further research is needed to fully understand their potential and limitations. One concern is the generation of human-like texts that resemble copyrighted works, raising intellectual property issues \cite{sun2023short}. Future work could focus on developing LLM-based tools to detect copyright infringement by leveraging external copyright databases. Data privacy is another challenge, as LLMs are trained on extensive datasets that may contain personal and sensitive information. This raises concerns about unintentional disclosure or reconstruction of protected data, requiring compliance with data privacy legislation like the GDPR \cite{regulation2018general}. Potential solutions include providing prompts to remind LLMs to keep protected data private or fine-tuning them using external datasets without private information. Bias and fairness are also concerns in LLMs, as they may learn and perpetuate biases from training data. This can affect decision-making in legal contexts, such as legal argument development or case outcome prediction. Addressing this issue may involve prompt-based guidances to correct biases or referencing external unbiased case databases. These areas warrant further investigation to ensure the responsible and ethical use of LLMs in the legal domain.

\subsection{Education}
 LLMs revolutionize education in various aspects, including healthcare research \cite{sallam2023utility}, medical education \cite{hisan2023chatgpt,khan2023chatgpt,o2022open}, library management \cite{lund2023chatting,verma2023novel}, journal and media education \cite{pavlik2023collaborating}, engineering education \cite{qadir2022engineering}, academia \cite{m2022exploring,islam2023opportunities}, autodidactic education \cite{firat2023chat}, and higher education \cite{zhangpreparing,rudolph2023chatgpt}. The introduction of LLMs benefits both students and teachers \cite{kasneci2023chatgpt,baidoo2023education}: for students, the utilization of LLMs facilitates the training of question-asking skills \cite{abdelghani2022gpt}, engages students in solving real-world problems \cite{zhai2022chatgpt,malinka2023educational}, enhances learning pharmacology and algebra as a self-studying instrument \cite{nisar2023chatgpt,pardos2023learning}. For teachers or faculties, LLMs have great potentials to assist in teaching skills such as mechanical writing \cite{bishop2023computer} and reducing teaching workloads such as the quality assessment of short answer questions \cite{moore2022assessing} and course design \cite{gupta2023chatgpt}. Despite the potential benefits of LLMs, many existing works  demonstrate the limitations of LLMs such as the difficulty in understanding advanced subjects \cite{frieder2023mathematical} and failure to achieve difficult problems \cite{shakarian2023independent}. Some preliminary investigations utilized promoting techniques to improve the performance of LLMs \cite{lievin2022can}. This will inspire more future works to explore domain specification techniques for education, which is still an open research area. Existing research works in this area can be classified into two categories: assessing LLMs' performance on various education tasks and addressing concerns raised by LLMs' introduction to educational ethics.
\subsubsection{Capability Assessment}
A significant area of research examines the effectiveness of LLMs in various subjects, aiming to evaluate their potential as learning assistants. The debate over the capabilities of LLMs on medical exams remains a hot topic in the field. While some case studies suggest that LLMs performed worse than students in medical exams \cite{huh2023chatgpt,fijavcko2023can,wang2023chatgpt}, other experiments indicate their promising performance on medical exams, either through the chain of thought prompting \cite{lievin2022can} or without additional fine-tuning \cite{gilson2023does,kung2023performance,mbakwe2023chatgpt}. A similar controversy also exists in mathematics, where the performance of ChatGPT varies considerably depending on the problem requirement \cite{shakarian2023independent,zong2022solving}. Furthermore, some studies have shown that the mathematical capabilities of ChatGPT fall below those of average math graduate students \cite{frieder2023mathematical}. In contrast, Kortemeyer, Bordt, and Luxburg found that ChatGPT can pass undergraduate-level exams in physics and computer science \cite{bordt2023chatgpt,kortemeyer2023could}. Bommarito et al. have also demonstrated ChatGPT's improved performance on the CPA examination \cite{bommarito2023gpt}.

In contrast to most assessments on the exam performance of LLMs, Tack and Piech investigated the pedagogical ability of GPT-3 and discovered that it was quantifiably worse than real teachers on several pedagogical dimensions \cite{tack2022ai}. Despite these mixed results, the potential of LLMs to assist students in their learning remains a significant area of research. By providing instant feedback and personalized learning experiences, LLMs can help students identify their strengths and weaknesses and gain a better understanding of the material. Moreover, they can aid teachers in delivering personalized instruction, developing course content, and reducing the burden of administrative tasks.
\subsubsection{Educational Ethics}
LLMs offer many possibilities for enhancing students' learning experiences, but they also present ethical challenges and risks. One significant risk is scientific misconduct, where students could use LLMs such as GPT-3 to generate convincing and seemingly original texts without additional learning or effort \cite{dehouche2021plagiarism}. This potential for academic dishonesty could result in serious repercussions for both students and educational institutions. Additionally, students might use LLMs like ChatGPT to author their essays instead of composing them independently, undermining the core principles of education \cite{king2023conversation}. ChatGPT's capacity to think critically and produce highly realistic texts with minimal input further exacerbates this threat to educational integrity \cite{susnjak2022chatgpt}. Moreover, Khalil and Er noted that ChatGPT can create sophisticated, original texts that remain undetected by prominent plagiarism detection tools, heightening the risk of academic misconduct \cite{khalil2023will}. Several papers propose potentially effective strategies to combat plagiarism and dishonesty. For instance, designing open-ended assessments that encourage originality and creativity can promote academic honesty \cite{cotton2023chatting}. Incorporating oral presentations, group projects, and hands-on activities requiring students to demonstrate their knowledge and skills in a more engaging, interactive way can also help foster honesty and reduce reliance on LLMs \cite{king2023conversation}. By deploying such strategies, educators can cultivate an environment that encourages originality, creativity, and academic integrity, while still leveraging the advantages of LLMs.

\subsubsection{Future Research Opportunities and Challenges}
Specializing LLMs in the education domain presents numerous opportunities for future research and innovation. From the perspective of \textit{external resource augmentation}, LLMs can be utilized to search for customized educational content and resources tailored to individual learners' needs, preferences, and abilities, facilitating more effective and personalized learning experiences. From the perspective of \textit{prompt crafting}, LLMs can be tailored to generate step-by-step explanations for the user provided question. In terms of \textit{model fine-tuning}, a specialized LLMs can be employed as an automatical homework grader of one specific subject. Additionally, LLMs can also be fine-tuned to detect potential plagiarism and academic misconduct. 


%While LLMs have been extensively studied in various subjects, their understanding of specialized subjects such as graduate-level mathematics and intellectual property law lags behind their understanding of preliminary subjects such as elementary mathematics. Therefore, it would still be necessary to develop. With the increasing power of LLMs, further research is needed to explore their potential role in enhancing students' learning experiences and reducing teachers' workloads. For example, LLMs can generate personalized course materials for students based on prompts in the form of homework assessments and exam feedback, helping students to learn more effectively. Additionally, LLMs can be used in conjunction with external thesis databases to help faculties detect potential plagiarism and academic misconduct.


\subsection{Human Computer Interaction}
\begin{wrapfigure}[10]{r}{3cm}
\vspace{-15pt}
\begin{center}
    \includegraphics[width=0.20\textwidth]{figures/loona.png}
  \end{center}
  \caption{Loona, a pet robot integrated with ChatGPT.} 
  % \footnote{https://keyirobot.com/pages/loonadetail}
  % }
% \vspace{-5pt}
\end{wrapfigure}
The advent of LLM opened the door of human-AI collaboration in diverse directions for human-computer interaction (HCI) systems. LLM can be integrated with a lot of HCI systems. Currently, KEYi Technology has integrated ChatGPT with their pet robot ``Loona''\footnote{https://keyirobot.com/pages/loonadetail}. HCI systems can be dependent on single or multiple-channel interactions of sensory input/output modalities. To utilize the LLM there needs a process of language understanding so that, cross-modal input can be utilized with LLM. The response from the LLM can be combined with the modal-oriented model blocks to do the domain adaptation for the LLM. Among many tasks, the mainstream tasks of HCI revolve around 1) speech and dialogue related tasks and 2) vision related tasks.
%A common generic approach has been shown in Figure \ref{fig: HCI}. Among many tasks, the mainstream tasks of HCI revolve around 1) speech and dialogue related tasks and 2) vision related tasks.
% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=.90\textwidth]{figures/LLM_HCI.pdf}
%     \caption{Generic approach for LLM adaptation for HCI applications. The first step is to understand the intention of the multi-modal input. After the natural language understanding, prompt engineering can help to get a better response from the LLM. Eventually, the response can be used with the modal-oriented models to make an improved HCI system.}
%     \label{fig: HCI}
%     \end{figure*}

\subsubsection{Speech and Dialogue Related Tasks}
This field of research faces obstacles due to a lack of large-scale text-audio matching and sophisticated waveform data. In a survey, the authors categorized the tasks in seven speech-related domains including automatic speech recognition (ASR), neural speech synthesis, speech translation (ST), speech paralinguistics, speech enhancement and separation, spoken dialogue systems, and multi-modal application \cite{latif2023transformers}. Aside from this, LLMs may be used for data augmentation, as Chen et al. \cite{chen2023places} employed LLMs to produce synthetic social conversations spanning a variety of everyday themes, such as school life and relationships. Additionally, the toxicity of the LLM-generated substance poses a problem when it comes to dealing with people. Meade et al. attempted to lessen bias and toxicity in responses provided by neural-based chatbots by employing a retrieval-based framework where they graded a variety of alternative solutions based on what they refer to as safety demonstrations \cite{meade2023using}. Sometimes the response generated for the dialogue system becomes inappropriate due to weak dialogue history management. This issue was solved by using a three-component system (style, reference resolution, and response generation) by Kinouchi and Kitaoka \cite{kinouchi2022response}. Here they used the Japanese Text-to-Text Transfer Transformer (T5), and the Japanese GPT-2 based response generation model. In another work, high-quality audio generation was accomplished by mapping the audio to the semantic tokens and acoustic tokens \cite{borsos2022audiolm}. This semantic tokens generation can be benefited from a large language model. A preliminary analysis on the spoken conversation corpus by \cite{zorrilla2021audio} demonstrated that audio embeddings may indeed encode meaningful acoustic information and utilize it to learn improved dialogue policies when paired with GPT-2 transformer-based neural dialogue policies. Transfer learning is also pursued for dialogue systems to utilize the LLM especially when the domain data is insufficient \cite{shalyminov2020hybrid}.

\subsubsection{Vision Related Tasks}
A vast quantity of data is used to train large language models. Subsequent research works have investigated the transfer of these pretrained large language models in other visual tasks. One way is to focus on the weight initialization of the model \cite{luo2022vc, chen2022visualgpt}. In  VC-GPT \cite{luo2022vc}, authors utilized two pre-trained models visual encoder (CLIP-ViT) and language decoder (GPT2) to initialize the primary blocks of the model. Then used a self-ensemble cross-modal fusion module to connect those blocks for image captioning tasks. In another work, VisualGPT \cite{chen2022visualgpt} connected the multi-level visual features with the knowledge from pretrained language model via a self-resurrecting attention mechanism. Nevertheless, for challenging tasks such as storytelling with image data, there is a concern that this direct transfer approach may suffer from a mismatch between visual specificity and language fluency because they are typically trained independently from the enormous corpus of visual and text data with no common ground. The authors in \cite{yu2021transitional} proposed TAPM that included a simple pretext task as an adaptation process that harmonizes the visual encoding and language modeling before optimizing the target objective. Another popular approach is few-shot learning. One work in few-shot learning is FLamingo \cite{alayrac2022flamingo}, a family of Visual
Language Models (VLMs), which ingest images or videos as input. By bridging the powerful pretrained models it can handle sequences of arbitrarily interleaved visual and textual data which enables in-context few-shot learning capabilities of multimodal tasks (generation, classification). In another work \cite{zhang2023prompt}, the model CaFo followed the cascade paradigm to incorporate diverse prior knowledge of various pretraining models for better few-shot learning. The pretrained LLM can be used to customize the prompt for the model. In \cite{pratt2022does}, first, they used the LLM-prompts (filled with class names) to generate image-prompts (descriptions for class categories). At later stage, they used these image-prompts to do the zero-shot image classification with the help of open vocabulary models.

\subsubsection{Future Research Opportunities}
When mobility, memory, and interaction time are taken into account, LLM-adapted human-computer interaction keeps being an important arena for cross-domain research. We have already seen the application of delivery robots in different industries. Yet developing a cost-effective, amicable, curious, behavioral constraint HCI system needs research in commonsense reasoning, large vocabulary continuous speech recognition, word spotting, lip-reading, eye-tracking, gesture recognition, handwriting recognition, consistent information response, visual question answering, etc.

\subsection{Software Engineering}
With the development of AI, the pair programming paradigm led to coin the term ``AI pair programmer''. And the LLM's capability to respond with different types of prompt crafting brought huge possibilities for using LLM as a compelling and promising component for software developers. Moreover, pre-trained LLMs can outperform the non-pre-trained model whether it is code understanding or code generation tasks \cite{zeng2022extensive}. The ongoing research can be diversified into two broader perspectives. Whether one group is trying to use a generalized LLM and the other group is more focused on using the LLM trained on code (LLMC).

\subsubsection{Generalized LLM}
An early study on GPT-3 proved the hypothesis  that AI-generated code can reduce the software production time \cite{narasimhan2021cgems}. But still, generalized LLM's performance is not promising in software development. For example, in the study \cite{jalil2023chatgpt}, ChatGPT faced difficulties with low-resource or distant language and was able to answer only 37.5\% correctly. Despite this, dialogue-based LLMs can still be a promising aid in solving programming exercises in the life sciences, particularly in the field of bioinformatics \cite{piccolo2023many}. With expert-drafted codebooks, GPT-3 performance can be improved substantially compared to expert-coded result \cite{xiao2023supporting}. Another way to boost performance is using multiple LLMs to distribute the workloads. By following a self-collaborating framework, three ChatGPT roles (i.e., analyst, coder, and tester) can improve the traditional coding generation of LLMs \cite{dong2023self}.

\subsubsection{LLM Trained on Code}
Large language models trained on code (LLMC) are the specialized versions of LLM trained on code, such as GPT-J-6B \cite{wang2021gpt}, GPT-Neo \cite{black2021gpt}, Codex (can be applied to almost all programming tasks) \cite{chen2021evaluating}, Alphacode (problems that require deeper reasoning) \cite{li2022competition}. There are many studies on LLM-based code completion frameworks focusing on cost reduction \cite{zhang2022diet}, security implication \cite{pearce2021can}, code explanation \cite{sarsa2022automatic} or potential extension in different domains (for example, reverse engineering \cite{pearce2022pop}, programming syntax error \cite{phung2023generating} etc.). By utilizing the Codex, the model CodexDB can process the SQL queries. They utilized the DB catalog and text-to-SQL methods to make the SQL query from the natural language instruction \cite{trummer2022codexdb}. The Codex can also be used to generate documentation-specific code examples by combining contexts from multiple sources (source code, documentation, and error logs from the compiler) \cite{khan2023combining}. Again, LLMCs are not limited to coding only. In a task where structure follows the code-like pattern (meaning representation \cite{shin2021few}), LLMCs can follow the same performance as LLM.

\subsubsection{Future Research Opportunities}
The LLM's semantic understanding from the given prompt is not identical to the human level. It can lead to producing different codes from logically the same but semantically different prompts \cite{li2022cctest}. Moreover, program synthesis also needs to make sure of the performance, security, licensing attribution, and multi-modal specifications \cite{jain2022jigsaw}. On the other hand, LLM updates can lead to producing inconsistent code for the same prompt \cite{fakhoury2023towards}. So, although promising, the adaptation of LLM still requires further advancement before it can be dependably used for software development in various contexts including code summarization, code repair, code translation, code generation, code search, program understanding, program debugging (i.e., detection, localization, and repair), code explanations, etc.

\subsection{Cybersecurity}
Cybersecurity involves protecting computer systems and networks from unauthorized access, use, disclosure, disruption, modification, or destruction. It includes measures like encryption, firewalls, antivirus software, access control, intrusion detection, and incident response. The main objective of cybersecurity is to ensure the confidentiality, integrity, and availability of digital assets and to prevent cyber attacks, such as phishing, malware, and ransomware. Cybersecurity is crucial for individuals, businesses, and governments as digital technologies become more widespread and cybercrime becomes a greater threat. Pretrained language models, like BERT, have been used in cybersecurity research. CyberBERT, proposed by Paul et al., is a BERT-based language model that identifies cyberbullying \cite{paul2022cyberbert}. SecureBERT, a BERT-based cybersecurity language model developed by Aghaei et al., captures text connotations used in automated security measures for critical cybersecurity tasks \cite{aghaei2023securebert}. While research on using LLMs for cybersecurity is still emerging, some studies have explored the potential consequences of cybercrimes using LLMs and how they can be developed to combat cybersecurity threats.
\subsubsection{Cyber Attacks}
LLMs like ChatGPT present dual cybersecurity implications \cite{shen2023chatgpt}. They can generate code emulating viruses, demonstrated by McKee and Noever's use of ChatGPT in creating virus-like codes with properties such as duplication and modification through the MITRE ATT\&CK framework \cite{mckee2022chatbots}. Conversely, LLMs can be weaponized for malicious purposes like crafting sophisticated phishing emails. Karanjai's exploration revealed LLMs' capability to generate hard-to-detect phishing emails, with effectiveness contingent on LLMs and training data \cite{karanjai2022targeted}. This underscores the need for distinguishing machine-generated emails from human ones and mitigating LLM misuse.

\subsubsection{Cyber Protection}
LLMs are predominantly researched for cyber attack protection measures. Akbar et al. developed a RoBERTa-based tool matching attack and defensive techniques for timely and effective threat response \cite{akbar2022knowledge}. Hewett and Matthew utilized GPT-3 to produce plausible replies to Advance Fee Fraud emails, disrupting fraudulent activities \cite{hewett2022developing}. LLMs' potential in zero-shot vulnerability repair was examined by Pearce et al., though challenges exist in generating correct code \cite{pearce2022examining}. Cambiaso and Luca explored ChatGPT for engaging scammers in futile interactions, effectively wasting their time and resources \cite{cambiaso2023scamming}. Thus, despite misuse concerns, LLMs are primarily seen as cybersecurity shields against attacks.

\subsubsection{Future Research Opportunities}
While some previous works have demonstrated the impressive ability of LLMs to carry out cyber attacks such as logic bombs and obfuscated worms \cite{shen2023chatgpt, mckee2022chatbots}, further studies are needed to investigate the performance of LLMs in other types of cyber attacks, such as Distributed Denial of Service (DDoS) \cite{lau2000distributed}, Man-in-the-middle (MitM) attacks \cite{bhushan2017man}, and zero-day attacks \cite{bilge2012before}. These studies can help researchers gain a more comprehensive understanding of the strengths and weaknesses of LLMs for cyber attacks and can inform the development of cybersecurity protection measures. It is worth noting that existing cybersecurity measures are often specialized and may not be effective against all types of threats \cite{cambiaso2023scamming}. This may motivate cybersecurity experts to investigate how LLMs trained to tackle a specific type of cyber attack can be adapted to other types of attacks. This could potentially be addressed by using prompts that describe common characteristics of cyber attacks in terms of dangers and consequences of cybersecurity vulnerability, in order to learn unified embedding representations of cyber attacks.
